Foncteur de Picard d'un champ alg\'ebrique

In this article we study the Picard functor and the Picard stack of an algebraic stack. We give a new and direct proof of the representability of the Picard stack. We prove that it is quasi-separated, and that the connected component of the identity is proper when the fibers of the stack are geometrically normal. We study some examples of Picard functors of classical stacks. In an appendix, we review the lisse-etale cohomology of abelian sheaves on an algebraic stack.

==> macros.tex <==
%********************* commandes ****************************
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\beqn}{\begin{eqnarray*}}
\newcommand{\eeqn}{\end{eqnarray*}}
\newcommand{\disp}{\displaystyle}
\newcommand{\flechen}[3]{%
\xymatrix{
{#1} \ar[r]^-{#2} & {#3} }}
%\def\cartesien{%
%        \ar@{-}[]+R+<6pt,-1pt>;[]+RD+<6pt,-6pt>%
%        \ar@{-}[]+D+<1pt,-6pt>;[]+RD+<6pt,-6pt>%
%      }
\newcommand{\incl}[1][r]
      {\ar@<-0.2pc>@{^(-}[#1] \ar@<+0.2pc>@{-}[#1]}
%*********** Mots gras ****************
\newcommand{\dem}{{\bf D\'emonstration}}
\newcommand{\preuve}{{\bf Preuve}}
\newcommand{\rem}{{\bf Remarque }}
\newcommand{\lemme}{{\bf Lemme}}
\newcommand{\proposition}{{\bf Proposition}}
%\newcommand{\definition}{{\bf D\'efinition}}
\newcommand{\theo}{{\bf Th\'eor\`eme}}

%****************** Raccourcis mathématiques ****************
%********** Caractères usuels ***************
\def\C{{\mathbb C}}
\def\D{{\mathbb D}}
\def\F{{\mathbb F}}
\def\K{{\mathbb K}}
\def\M{{\rm M}}
\def\N{{\mathbb N}}
\def\P{{\mathbb P}}
\def\Q{{\mathbb Q}}
\def\R{{\mathbb R}}
\def\Z{{\mathbb Z}}
\def\Ac{{\mathcal A}}
\def\Bc{{\mathcal B}}
\def\Cc{{\mathcal C}}
\def\Fc{{\mathcal F}}
\def\Gc{{\mathcal G}}
\def\Hc{{\mathcal H}}
\def\Ic{{\mathcal I}}
\def\Lc{{\mathcal{L}}}
\def\Mc{{\mathcal M}}
\def\Nc{{\mathcal N}}
\def\Oc{{\mathcal O}}
\def\Pc{{\mathcal P}}
\def\Qc{{\mathcal Q}}
\def\Rc{{\mathcal R}}
\def\Sc{{\mathcal S}}
\def\Tc{{\mathcal T}}
\def\Uc{{\mathcal U}}
\def\Vc{{\mathcal{V}}}
\def\Zc{{\mathcal{Z}}}
\def\Ago{{\mathfrak A}}
\def\mgo{{\mathfrak m}}
\def\pgo{{\mathfrak p}}
\def\qgo{{\mathfrak q}}
\def\Sgo{{\mathfrak S}}
\def\gm{{\mathbb G}_{\rm{m}}}
\def\mun{{\mu}_n}
\def\bgm{{\rm B}{\mathbb G}_{\rm{m}}}
\def\bmun{{\rm B}\mun}
\def\bmunfppf{({\rm B}\mun)_{{\rm fppf}}}
\def\eps{\varepsilon}
\def\fleche{\longrightarrow}
\def\inj{\hookrightarrow}
\def\tend{\rightarrow}
\def\ov{\overline}
%***** Fonctions ou opérateurs usuels ******
\newcommand{\cartesien}{\ar@{}[dr]|{\square}}
\def\FlecheNE{\rotatebox[origin=c]{45}{\ensuremath \Rightarrow}}


\newcommand{\turndown}[1]{\rotatebox[origin=c]{270}{\ensuremath#1}}
\newcommand{\hookdownarrow}{\turndown{\hookrightarrow}}


\def\lind{\lim_{\longrightarrow}}
\def\lpro{\lim_{\longleftarrow}}
\def\ln{\hbox{\rm ln}\,}
\def\com{\hbox{\rm com}\,}
%\def\mod{\hbox{\rm mod}\,}
\def\rg{\hbox{\rm rg}\,}
\def\pr{{\rm pr}}
\def\Ker{\hbox{\rm Ker}\,}
\def\Coh{\hbox{${\mathfrak{Coh}}$}\,}
\def\Mod{\hbox{\rm Mod}}
\def\Ab{\hbox{\rm Ab}}
\def\Aut{\hbox{\rm Aut}}
\def\Auts{\hbox{\rm \underline{Aut}}}
\def\Stab{\hbox{\rm Stab}\,}
\def\Ind{\hbox{\rm Ind}\,}
\def\Isom{\hbox{\rm Isom}}
\def\Isoms{\hbox{\rm \underline{Isom}}}
\def\fIsom{{\mathcal I\!som}\,}
\def\fAut{{\mathcal Aut}\,}
\def\rang{\hbox{\rm rang}\,}
\def\pgcd{\hbox{\rm pgcd}\,}
\def\diag{\hbox{\rm diag}}
\def\div{\hbox{\rm div}}
\def\rot{\hbox{\rm rot}}
\def\tr{\hbox{\rm tr}\,}
\def\o{\hbox{\rm o}}
\def\ob{\hbox{\rm ob}\,}
\def\cosq{\hbox{\rm cosq}}
\def\sq{\hbox{\rm sq}}
\def\O{\hbox{\rm O}}
\def\l{{l}}
\def\Im{\hbox{\rm Im}\,}
\def\Id{{\rm Id}}
\def\id{\hbox{\rm id}}
\def\Re{\hbox{\rm Re}\,}
\def\Der{\hbox{\rm Der}\,}
\def\Com{\hbox{\rm Com}\,}
\def\Hom{\hbox{\rm Hom}}
\def\Ext{\hbox{\rm Ext}\,}
\def\fHom{{\mathcal{H}om}\,}
\def\fExt{{\mathcal{E}xt}\,}
\def\grad{{\overrightarrow{\textrm{grad}}}\,}
%\def\grad{\hbox{{\rm grad}}\,}
\def\Spec{{\rm Spec}\,}
\def\Ens{\hbox{\rm Ens}\,}
\def\pgcd{\hbox{\rm pgcd}\,}
\def\ch{\hbox{\rm ch}\,}
\def\sh{\hbox{\rm sh}\,}
\def\Arg{\hbox{\rm Arg}\,}
\def\Card{\hbox{\rm Card}\,}
\def\GL{\hbox{\rm GL}\,}
\def\GLc{{\mathcal{G\!L}}}
\def\SL{\hbox{\rm SL}\,}
\def\t{|\!|\!|}
\def\ss{\scriptstyle}
\def\ms{\medskip}
\def\rp{{\sl resp~:~}}
\def\overcircle{\,\,{}^{{}^{{}^{\circ}}}\!\!\!\!}
\def\di#1#2{_{\hbox{\vbox{\hbox{$\ss#1$}%
\vskip-1.5mm%
\hbox{$\ss#2$}}}}}

%%%*********************Macros plus evoluees********************
%
%
\newcommand{\eme}[1]{${#1}^{\textrm{ème}}$}
\newcommand{\iem}[1]{${#1}^{\textrm{ième}}$}
% Faire des fractions qui ont toujours la bonne taille
% Exemple : $\f{1}{2}$, mais aussi $x^{\f{3}{2}}$.
\newcommand{\f}[2]{{\ensuremath{\mathchoice%
%	{\dfrac{#1}{#2}}
%       {\dfrac{#1}{#2}}
	{\frac{#1}{#2}}
	{\frac{#1}{#2}}
	}}}

%%% Faire une fleche longue pour une limite.
\newcommand{\tv}[1]{\ensuremath{\xrightarrow[#1]{}}}
	% Exemple : $f(x) \tv{x\to 0} 1$
\newcommand{\tvn}{\ensuremath{\tv{n \to \infty}}}
	% Exemple : $u_n \tvn \pi$

%%% Faire des intégrales qui ont toujours la bonne taille.
% Ne jamais utiliser \int !
\newcommand{\Int}[2]{\ensuremath{\mathchoice%
	{\displaystyle\int_{#1}^{#2}}
	{\displaystyle\int_{#1}^{#2}}
	{\int_{#1}^{#2}}
	{\int_{#1}^{#2}}
	}}

%%% Les éléments différentiels dans les intégrales.
% Exemples : $\Int{0}{1} f(t) \dt$
% $\f{\dd \Phi}{\dd t}$ % Attention, ne pas mettre {\dt} au dénominateur.
\newcommand{\dd}{\ensuremath{\text{d}}}
\newcommand{\dt}{\ensuremath{\:\dd t}}
\newcommand{\dx}{\ensuremath{\:\dd x}}
\newcommand{\dy}{\ensuremath{\:\dd y}}
\newcommand{\dz}{\ensuremath{\:\dd z}}
\newcommand{\du}{\ensuremath{\:\dd u}}
\newcommand{\dv}{\ensuremath{\:\dd v}}
\newcommand{\dr}{\ensuremath{\:\dd r}}
\newcommand{\dS}{\ensuremath{\,\dd\!\vect{S}}}

\newcommand{\trinorme}[1]{\ensuremath{|\hskip -1 pt|\hskip -1 pt| #1%
	|\hskip -1 pt|\hskip -1 pt|}}
	% Y'a vraiment des gens qui font des maths bizarres.
\newcommand{\Dp}[2]{\ensuremath{\frac{\partial#1}{\partial#2}}} 
	% Dérivée partielle : « D rond f sur D rond t » s'écrit $\Dp{f}{t}$~.

%%% Faire des listes de façon pratique.
\newcommand{\xlist}[2]{\ensuremath{\left({#1}_1,\ldots,{#1}_{#2}\right)}}

\newcommand{\nlist}[1]{\xlist{#1}{n}}
\newcommand{\mlist}[1]{\xlist{#1}{m}}
\newcommand{\plist}[1]{\xlist{#1}{p}}
\newcommand{\rlist}[1]{\xlist{#1}{r}}
	% Exemple : La famille $\nliste{e}$ est libre.

\newcommand{\intn}[2]{\ensuremath{%
        \left[\!\left[ \, #1 \,;\, #2 \,\right]\!\right]}}
	% Pour les intervalles d'entiers.
	% Exemple : $\forall k \in \intn{0}{n-1} \quad |u_k| < 1$.

%% Pour les matrices
\newcommand{\udots}{\ensuremath{\hskip 2pt \raisebox{1pt}{.} \hskip 1pt%
        \raisebox{4pt}{.} \hskip 1pt \raisebox{7pt}{.} \hskip 2pt}}
	% up-dots, le symérique de \ddots sur la diagonale.
\newcommand{\trans}[1]{\ensuremath{\sideset{^t}{}%
        {\mathop{\mathstrut #1}}}}
	% La transposée d'une matrice : $\trans{A}$.
\newenvironment{matrice}%
	{\begin{pmatrix}}%
	{\end{pmatrix}}
	% Vu que c'est presque toujours celui-là qu'il nous faut...
\newenvironment{determinant}%
	{\begin{vmatrix}}%
	{\end{vmatrix}}
%% Des environnements tres pratiques !

\newenvironment{syst}[1][c]%
	{\ensuremath{\left \{ \hskip -1.5 mm \begin{array}{#1@{\ =\ }l}}}%
	{\end{array}\right.}
	% Exemple : $\begin{syst} a & b+2 \\ b & 1 \\ \end{syst}$ 
	% fait ce que l'on pense, ie met un signe égal avec des espaces de
	% et d'autre.

\newenvironment{varsyst}[1][r]%
	{\ensuremath{\left \{ \hskip -1.5 mm%
	 \begin{array}{#1@{\ }c@{\ }l}}}%
	{\end{array}\right.}
	% Pour les calculs qui font intervenir autre chose qu'un signe =,
	% par exemple \leq ou \geq ou \sim, quelque part.


\newenvironment{accolade}[1][c]%
	{\ensuremath{\left \{ \hskip -1.5 mm \begin{array}{#1@{\quad}l}}}%
	{\end{array}\right.}
	% Exemple : $f(x) = \begin{accolade} \bigskip
	%	\f{\sin x}{x} & \text{si } x\neq 0 \\
	%	1 & \text{sinon} \\
	%	\end{accolade}$
\newcommand{\fonction}[5]{%
        \ensuremath{#1\colon
        \left\{\hskip -1.5 mm                   %}
        \begin{array}{c@{\ }c@{\ }l}
        \medskip #2 & \longrightarrow & #3 \\
        #4 & \longmapsto & #5 \\
        \end{array}
        \right .
        }}
	% $\fonction{f}{\intoo{0}{\pinf}}{\intoo{-1}{\pinf}}{x}{\f{1}{x}-1}$
	% dessine la même chose que ce que l'on fait naturellement à la main :
	% le symbole f, suivi d'un ':', d'une accolade, puis sur deux
	% lignes l'ensemble de définition, d'arrivée, puis la variable et
	% l'expression de f(x).

\newcommand{\quotient}[2]{
#1/#2}

\newcommand{\parmi}[2]{\left( \begin{array}{c}
#2\\ #1 
\end{array}\right)
}
\renewcommand{\parmi}[2]{\binom{#2}{#1}
}


==> packusu.tex <==
\usepackage[T1]{fontenc}
\usepackage[latin1]{inputenc}
%\usepackage{dsfont}\let\mathbb\mathds
\usepackage[french]{babel}
%\usepackage{verbatim}
\usepackage{latexsym}
\usepackage{amsfonts}
\usepackage{amstext}
\usepackage{amsmath}
\usepackage{graphicx}
%\usepackage{rotating}
\usepackage[all,dvips]{xy}
\input xy
\xyoption{all}
\usepackage{amssymb,euscript,multicol,graphicx}
\usepackage[ec]{aeguill}       %Ca c'est pour que les pdf soient beaux....
\usepackage{delarray, fancyhdr}



==> sectionnement.tex <==
%**** Sectionnement : théorèmes, corollaires, etc... ********
\newtheorem{cor}[subsection]{Corollaire}
\newtheorem{souscor}[subsubsection]{Corollaire}
\newtheorem{prop}[subsection]{Proposition}
\newtheorem{sousprop}[subsubsection]{Proposition}
\newtheorem{thm}[subsection]{Th\'eor\`eme}
\newtheorem{sousthm}[subsubsection]{Th\'eor\`eme}
\newtheorem{defi}[subsection]{D\'efinition}
\newtheorem{sousdefi}[subsubsection]{D\'efinition}
\newtheorem{lem}[subsection]{Lemme}
\newtheorem{souslem}[subsubsection]{Lemme}
\newtheorem{pptes}[subsection]{Propri\'et\'es}
\newtheorem{souspptes}[subsubsection]{Propri\'et\'es}
\newtheorem{remarque}[subsection]{Remarque}
\newtheorem{sousremarque}[subsubsection]{Remarque}
\newtheorem{exemple}[subsection]{Exemple}
\newtheorem{sousexemple}[subsubsection]{Exemple}
\newtheorem{conjecture}[subsection]{Conjecture}
\newtheorem{sousconjecture}[subsubsection]{Conjecture}

%**** Environnements : demonstrations, etc... ***************
\newenvironment{demo}{{\bf D\'emonstration}}{$\square$ \vskip .3cm}
\newenvironment{democ}[1]{{\bf D\'emonstration #1}}{$\square$ \vskip .3cm}
\newenvironment{etape}[1]{$\bullet$ \emph{#1}\\}{\vskip .2cm}
\newenvironment{etapefinale}[1]{$\bullet$ \emph{#1}\\}{}
%\newenvironment{exemple}{{\bf Exemple}}{\vskip .2cm}
%\newenvironment{remarque}
%  {\addtocounter{subsection}{1}\noindent{\bf Remarque \thesubsection\ \ }}
%  {\vskip .2cm}
%\newenvironment{sousremarque}
%  {\addtocounter{subsubsection}{1}\noindent{\bf Remarque \thesubsubsection\ \ }}
%  {\vskip .2cm}
%\renewtheorem{remarque}{\rm}{}

